Q-PART: Quasi-Periodic Adaptive Regression with Test-time Training for Pediatric Left Ventricular Ejection Fraction Regression

In this work, we address the challenge of adaptive pediatric Left Ventricular Ejection Fraction (LVEF) assessment. While Test-time Training (TTT) approaches show promise for this task, they suffer from two significant limitations. Existing TTT works are primarily designed for classification tasks rather than continuous value regression, and they lack mechanisms to handle the quasi-periodic nature of cardiac signals. To tackle these issues, we propose a novel \textbf{Q}uasi-\textbf{P}eriodic \textbf{A}daptive \textbf{R}egression with \textbf{T}est-time Training (Q-PART) framework. In the training stage, the proposed Quasi-Period Network decomposes the echocardiogram into periodic and aperiodic components within latent space by combining parameterized helix trajectories with Neural Controlled Differential Equations. During inference, our framework further employs a variance minimization strategy across image augmentations that simulate common quality issues in echocardiogram acquisition, along with differential adaptation rates for periodic and aperiodic components. Theoretical analysis is provided to demonstrate that our variance minimization objective effectively bounds the regression error under mild conditions. Furthermore, extensive experiments across three pediatric age groups demonstrate that Q-PART not only significantly outperforms existing approaches in pediatric LVEF prediction, but also exhibits strong clinical screening capability with high mAUROC scores (up to 0.9747) and maintains gender-fair performance across all metrics, validating its robustness and practical utility in pediatric echocardiography analysis.

==> table/algorithms.tex <==
\begin{algorithm}[t]
	\caption{Test-time Training for Quasi-Period Network}
	\label{alg:ttt_qpn}
	\begin{algorithmic}[1]
		\Require Training data $\mathcal{D}_{train} = \{(\boldsymbol{x}_i, y_i)\}_{i=1}^N$, test sample $\boldsymbol{x}_{test}$
		\Ensure Adapted model parameters $\theta$
		
		\State // Training Phase
		\For{each training iteration}
		\State $\boldsymbol{z} \gets \text{Enc}(\boldsymbol{x})$ \Comment{Initial feature extraction}
		
		\State // Periodic Component
		\State $f, \phi, b, v \gets p(\boldsymbol{z})$ \Comment{Extract periodic parameters}
		\State $\boldsymbol{\hat{z}}^{period} \gets \cos(2\pi(ft-\phi)) + \sin(2\pi(ft-\phi)) + vt + b$
		
		\State // Aperiodic Component
		\State $\boldsymbol{z}' \gets \boldsymbol{z} - \boldsymbol{\hat{z}}^{period}$ \Comment{Residual features}
		\State $\boldsymbol{V}(t) \gets \text{CubicSpline}(\boldsymbol{z}'_t)$ \Comment{Continuous path}
		\State $\boldsymbol{\hat{z}}^{aperiod} \gets \boldsymbol{z}'_0 + \int_0^T f_{\theta}(\boldsymbol{\hat{z}}^{aperiod}_t, t) d\boldsymbol{V}(t)$
		
		\State // Loss Computation
		\State Calculate training loss $\mathcal{L}_{total}$ using Eq. \ref{eq:train_total}
		\State Update model parameters
		\EndFor
		
		\State // Test-time Training Phase
		\For{each test sample $\boldsymbol{x}_{test}$}
		\State // Generate Augmented Samples
		\State $\{\boldsymbol{x}_{test}^k\}_{k=1}^K \gets \mathcal{T}_{aug}(\boldsymbol{x}_{test})$
		
		\For{each adaptation iteration}
		\For{$k = 1$ to $K$}
		\State Forward pass $\boldsymbol{x}_{test}^k$ through network
		\State Compute predictions $\hat{y}_k$
		\EndFor
		
		\State // Compute Test-time Losses
		Calculate test-time loss $\mathcal{L}_{test}$ using Eq. \ref{eq:loss_test}
		
		\State // Differential Adaptation
		\State Update periodic BN parameters with small learning rate
		\State Update aperiodic BN parameters with large learning rate
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}
